Multi-Patch Prediction: Adapting LLMs for Time Series Representation Learning

In this study, we present aLLM4TS, an innovative framework that adapts Large Language Models (LLMs) for time-series representation learning. Central to our approach is that we reconceive time-series forecasting as a self-supervised, multi-patch prediction task, which, compared to traditional contrastive learning or mask-and-reconstruction methods, captures temporal dynamics in patch representations more effectively. Our strategy encompasses two-stage training: (i). a causal continual pre-training phase on various time-series datasets, anchored on next patch prediction, effectively syncing LLM capabilities with the intricacies of time-series data; (ii). fine-tuning for multi-patch prediction in the targeted time-series context. A distinctive element of our framework is the patch-wise decoding layer, which departs from previous methods reliant on sequence-level decoding. Such a design directly transposes individual patches into temporal sequences, thereby significantly bolstering the model's proficiency in mastering temporal patch-based representations. aLLM4TS demonstrates superior performance in several downstream tasks, proving its effectiveness in deriving temporal representations with enhanced transferability and marking a pivotal advancement in the adaptation of LLMs for time-series analysis.

==> tables/representation_full.tex <==
\begin{table*}[!htbp]
\centering
    \vspace{-2mm}
    \caption{
    Representation learning methods comparison. 
    \textit{NPP} implies conducting alignment stage 1, next-patch casual pre-training, and stage 2, multi-patch decoding. 
    % 
    \textit{MPD} implies conducting alignment stage 2, multi-patch representation optimization, and patch-level decoding.
    % % 
    \textit{Masking-$\ast\%$} implies replacing the next-patch casual pre-training with masking-patch pre-training in stage 1 of masking ratio $\ast\ast\%$~(\textit{Masking} in PatchTST denotes using default masking ratio $40\%$ as its origin paper). 
    % 
    \textit{SD} denotes using a huge sequence-level decoding layer instead of the patch-level layer.
    % 
    {\boldres{Red}}: the best, \secondres{Blue}: the second best.
    IMP. denotes the improvement on best results of \method{} compared to that of baselines.
    }
    \scalebox{0.56}{
        \begin{tabular}{cc|c|c|cccccccc|cccccccc|ccccccccc}
            \cline{2-28}
            &\multicolumn{2}{c|}{\multirow{2}{*}{Models}}& \multirow{2}{*}{IMP.}& \multicolumn{8}{c|}{\method{}}& \multicolumn{8}{c|}{PatchTST}&  \multicolumn{2}{c|}{\multirow{2}{*}{BTSF}}&\multicolumn{2}{c|}{\multirow{2}{*}{TS2Vec}}&\multicolumn{2}{c|}{\multirow{2}{*}{TNC}}&\multicolumn{2}{c}{\multirow{2}{*}{TS-TCC}}& \\
            \cline{5-20}
            &\multicolumn{2}{c|}{}& &\multicolumn{2}{c|}{NPP+MPD}& \multicolumn{2}{c|}{Masking-20+MPD}&\multicolumn{2}{c|}{Masking-40+MPD}&\multicolumn{2}{c|}{Masking-60+MPD}& \multicolumn{2}{c|}{NPP+MPD}& \multicolumn{2}{c|}{MPD}& \multicolumn{2}{c|}{Masking+SD}& \multicolumn{2}{c|}{Masking+MPD}& \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} & \\
            \cline{2-28}
            &\multicolumn{2}{c|}{Metrics}& MSE &MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE&MSE&MAE\\
            \cline{2-28}
            &\multirow{5}*{\rotatebox{90}{ETTh1}} & 24  & 6.52$\%$ &\boldres{0.301} & \boldres{0.362}& 0.417 & 0.435 & 0.441 & 0.447 & 0.463 & 0.457 & 0.402 & 0.433 & 0.490 & 0.479 & 0.322 & 0.369 & 0.431 & 0.453 & 0.541 & 0.519 & 0.599 & 0.534 & 0.632 & 0.596 & 0.653 & 0.610 \\
            % 
            &\multicolumn{1}{c|}{}& 48 & xxx$\%$ &\boldres{0.343} & \boldres{0.377}& 0.418 & 0.437 & 0.422 & 0.439 & 0.429 & 0.442 & 0.401 & 0.432 & 0.482 & 0.476 & 0.354 & 0.385 & 0.437 & 0.467 & 0.613 & 0.524 & 0.629 & 0.555 & 0.705 & 0.688 & 0.720 & 0.693 \\
            % 
            &\multicolumn{1}{c|}{}& 168 & 6.21$\%$ &\boldres{0.393} & \boldres{0.415}& 0.436 & 0.448  & 0.437 & 0.449 & 0.441 & 0.451 & 0.416 & 0.441 & 0.478 & 0.478 & 0.419 & 0.424 & 0.459 & 0.480 & 0.640 & 0.532 & 0.755 & 0.636 & 1.097 & 0.993 & 1.129 & 1.044 \\
            % 
            &\multicolumn{1}{c|}{}& 336 & $7.20\%$ &\boldres{0.413} & \boldres{0.428}& 0.439 & 0.456  & 0.439 & 0.458 & 0.449 & 0.463 & 0.440 & 0.454 & 0.477 & 0.486 & 0.445 & 0.446 & 0.479 & 0.483 & 0.864 & 0.689 & 0.907 & 0.717 & 1.454 & 0.919 & 1.492 & 1.076 \\
            % 
            &\multicolumn{1}{c|}{}& 720 & $5.34\%$ &\boldres{0.461} & \boldres{0.462}& 0.475 & 0.485  & 0.479 & 0.490 & 0.502 & 0.499 & 0.500 & 0.485 & 0.516 & 0.517 & 0.487 & 0.478 & 0.523 & 0.508 & 0.993 & 0.712 & 1.048 & 0.790 & 1.604 & 1.118 & 1.603 & 1.206 \\
            \cline{2-28}			
        \end{tabular}
    }
\label{table::compare with self-sup}
\vspace{-5mm}
\end{table*}
